A First Detection of the Connected 4-Point Correlation Function of Galaxies Using the BOSS CMASS Sample

We present an $8.1\sigma$ detection of the non-Gaussian 4-Point Correlation Function (4PCF) using a sample of $N_{\rm g} \approx 8\times 10^5$ galaxies from the BOSS CMASS dataset. Our measurement uses the $\mathcal{O}(N_{\rm g}^2)$ NPCF estimator of Philcox et al. (2021), including a new modification to subtract the disconnected 4PCF contribution (arising from the product of two 2PCFs) at the estimator level. This approach is unlike previous work and ensures that our signal is a robust detection of gravitationally-induced non-Gaussianity. The estimator is validated with a suite of lognormal simulations, and the analytic form of the disconnected contribution is discussed. Due to the high dimensionality of the 4PCF, data compression is required; we use a signal-to-noise-based scheme calibrated from theoretical covariance matrices to restrict to $\sim$ $100$ basis vectors. The compression has minimal impact on the detection significance and facilitates traditional $\chi^2$-like analyses using a suite of mock catalogs. The significance is stable with respect to different treatments of noise in the sample covariance (arising from the limited number of mocks), but decreases to $4.7\sigma$ when a minimum galaxy separation of $14 h^{-1}\mathrm{Mpc}$ is enforced on the 4PCF tetrahedra (such that the statistic can be modelled more easily). The detectability of the 4PCF in the quasi-linear regime implies that it will become a useful tool in constraining cosmological and galaxy formation parameters from upcoming spectroscopic surveys.

==> old-discon-discussion.tex <==

We first consider the projection of the disconnected contributions onto the isotropic basis function.

To start, let us define the 4PCF in absolute coordinates as
\beq
    \zeta(\vx_0,\vx_1,\vx_2,\vx_3) &=& \av{\delta(\vx_0)\delta(\vx_1)\delta(\vx_2)\delta(\vx_3)}.
\eeq
This parametrization is over-complete (such that it contains more degrees-of-freedom than necessary), but useful. The disconnected piece is given by
\beq\label{eq: disconnected-piece}
    \zeta^{(\mathrm{disc})}(\vx_0,\vx_1,\vx_2,\vx_3) &=& \av{\delta(\vx_0)\delta(\vx_1)}\av{\delta(\vx_2)\delta(\vx_3)}+\text{2 perms.}
\eeq
Projecting onto the $N=3$ isotropic basis, one obtains the full 4PCF estimator (cf.\,\ref{eq: 4pcf-multiplet-estimator})
\beq\label{eq: estimator-absolute}
    \hat\zeta_{\ell_1\ell_2\ell_3}(r_1,r_2,r_3) &\equiv& \frac{1}{V}\int d\vx_0 d\vx_1 d\vx_2 d\vx_3 \,\delta(\vx_0)\delta(\vx_1)\delta(\vx_2)\delta(\vx_3)\P^*_{\ell_1\ell_2\ell_3}(\hx_{10},\hx_{20},\hx_{30})\\\nonumber &=&\frac{1}{V}(-1)^{\ell_1+\ell_2+\ell_3}\sum_{m_1m_2m_3}\tj{\ell_1}{\ell_2}{\ell_3}{m_1}{m_2}{m_3}\int \prod_{i=0}^{3}\left[d\vx_i\,\delta(\vx_i)\right]Y^*_{\ell_1m_1}(\hx_{10})Y^*_{\ell_2m_2}(\hx_{20})Y^*_{\ell_3m_3}(\hx_{30})
\eeq
where we have invoked ergodicity to replace the expectations by a spatial average and denoted $\vx_{ij}\equiv\vx_i-\vx_j$. Note that we have ignored the effects of binning for clarity. The expression \eqref{eq: estimator-absolute} is somewhat different to \eqref{eq: 4pcf-multiplet-estimator} since we are working in absolute coordinates; this is chosen to ensure proper treatment of the origin, $\vx_0$. In expectation, the disconnected component of \eqref{eq: estimator-absolute} gives
\beq
    \zeta^{(\mathrm{disc})}_{\ell_1\ell_2\ell_3}(r_1,r_2,r_3) &=&  \frac{1}{V}(-1)^{\ell_1+\ell_2+\ell_3}\sum_{m_1m_2m_3}\tj{\ell_1}{\ell_2}{\ell_3}{m_1}{m_2}{m_3}\int \prod_{i=0}^{3}\left[d\vx_i\right]\xi(\vx_0,\vx_1)\xi(\vx_2,\vx_3)\\\nonumber
    &&\,\times\,Y^*_{\ell_1m_1}(\hx_{10})Y^*_{\ell_2m_2}(\hx_{20})Y^*_{\ell_3m_3}(\hx_{30}) + \text{2 perms.}
\eeq
where we have written the 2PCF as $\xi(\vx_0,\vx_1) = \av{\delta(\vx_0)\delta(\vx_1)}$. If we assume $\xi(\vx_0,\vx_1)$ to depend only on $\vx_{10}\equiv\vx_1-\vx_0$ by homogeneity, we may switch variables to $\vx_1\rightarrow\hr_1\equiv\hx_{10}$ allowing separability:
\beq
    \zeta^{(\mathrm{disc})}_{\ell_1\ell_2\ell_3}(r_1,r_2,r_3) &=&  \frac{1}{V}(-1)^{\ell_1+\ell_2+\ell_3}\sum_{m_1m_2m_3}\tj{\ell_1}{\ell_2}{\ell_3}{m_1}{m_2}{m_3}\int d\hr_1\,\xi(\vr_1)Y^*_{\ell_1m_1}(\hr_1)\int d\vx_0d\vx_2d\vx_3\,\xi(\vx_2,\vx_3)\nonumber\\
    &&\,\times\,Y^*_{\ell_2m_2}(\hx_{20})Y^*_{\ell_3m_3}(\hx_{30}) + \text{2 perms.}
\eeq
Inserting estimators for $\xi(\vr_1)$ and $\xi(\vr_2,\vr_3)$ as spatial integrals over the overdensity field $\delta$, we obtain the estimator
\beq
    \hat\zeta^{(\mathrm{disc})}_{\ell_1\ell_2\ell_3}(r_1,r_2,r_3) &=&  (-1)^{\ell_1+\ell_2+\ell_3}\sum_{m_1m_2m_3}\tj{\ell_1}{\ell_2}{\ell_3}{m_1}{m_2}{m_3}\left[\frac{1}{V}\int d\vy\,d\hr_1\,\delta(\vy)\delta(\vy+\vr_1)Y^*_{\ell_1m_1}(\hr_1)\right]\\\nonumber
    &&\,\times\,\left[\frac{1}{V}\int d\vx d\hr_2d\hr_3\,\delta(\vx+\vr_2)\delta(\vx+\vr_3)Y^*_{\ell_2m_2}(\hr_2)Y^*_{\ell_3m_3}(\hr_3)\right]\,+\,\text{2 perms.}
\eeq
returning to relative variables. This is unbiased, in the sense that $\av{\hat\zeta_{\ell_1\ell_2\ell_3}^{(\mathrm{disc})}(r_1,r_2,r_3)} = \zeta_{\ell_1\ell_2\ell_3}^{(\mathrm{disc})}(r_1,r_2,r_3)$.\footnote{Strictly this is true only in the limit of infinite volume $V$, but unlikely to be a concern in practice.}

For convenience, we define
\beq
    \hat\xi_{\ell m}(r) &\equiv& \frac{1}{V}\int d\vx d\hr\,\delta(\vx)\delta(\vx+\vr)Y^*_{\ell m}(\hr) \\\nonumber
    \hat\xi_{\ell m \ell'm'}(r,r') &\equiv& \frac{1}{V}\int d\vx d\hr d\hr'\,\delta(\vx+\vr)\delta(\vx+\vr')Y^*_{\ell m}(\hr)Y^*_{\ell'm'}(\hr'),
\eeq
such that
\beq
    \hat\zeta_{{\ell_1\ell_2\ell_3}}^{(\mathrm{disc})}(r_1,r_2,r_3) &=& (-1)^{\ell_1+\ell_2+\ell_3}\sum_{m_1m_2m_3}\tj{\ell_1}{\ell_2}{\ell_3}{m_1}{m_2}{m_3}\\\nonumber
    &&\,\times\,\left[\hat\xi_{\ell_1m_1}(r_1)\hat\xi_{\ell_2 m_2\ell_3m_3}(r_2,r_3)+\hat\xi_{\ell_2m_2}(r_2)\hat\xi_{\ell_1 m_1\ell_3m_3}(r_1,r_3)+\hat\xi_{\ell_3m_3}(r_3)\hat\xi_{\ell_1 m_1\ell_2m_2}(r_1,r_2)\right]
\eeq
(writing the permutations out explicitly, assuming $r_1<r_2<r_3$), and an unbiased estimator for the \textit{connected} 4PCF is given by
\beq\label{eq: connected-4pcf-estimator}
    \hat\zeta_{\ell_1\ell_2\ell_3}^{(c)}(r_1,r_2,r_3) = \hat\zeta_{\ell_1\ell_2\ell_3}(r_1,r_2,r_3)-\hat\zeta^{(\mathrm{disc})}_{\ell_1\ell_2\ell_3}(r_1,r_2,r_3),
\eeq
where we use \eqref{eq: 4pcf-multiplet-factorized-estimator} to evaluate $\hat\zeta_{\ell_1\ell_2\ell_3}(r_1,r_2,r_3)$. Addition of radial binning to this expression is straightforward.
